Overcoming Catastrophic Forgetting via Direction-Constrained Optimization

This paper studies a new design of the optimization algorithm for training deep learning models with a fixed architecture of the classification network in a continual learning framework. The training data is non-stationary and the non-stationarity is imposed by a sequence of distinct tasks. We first analyze a deep model trained on only one learning task in isolation and identify a region in network parameter space, where the model performance is close to the recovered optimum. We provide empirical evidence that this region resembles a cone that expands along the convergence direction. We study the principal directions of the trajectory of the optimizer after convergence and show that traveling along a few top principal directions can quickly bring the parameters outside the cone but this is not the case for the remaining directions. We argue that catastrophic forgetting in a continual learning setting can be alleviated when the parameters are constrained to stay within the intersection of the plausible cones of individual tasks that were so far encountered during training. Based on this observation we present our direction-constrained optimization (DCO) method, where for each task we introduce a linear autoencoder to approximate its corresponding top forbidden principal directions. They are then incorporated into the loss function in the form of a regularization term for the purpose of learning the coming tasks without forgetting. Furthermore, in order to control the memory growth as the number of tasks increases, we propose a memory-efficient version of our algorithm called compressed DCO (DCO-COMP) that allocates a memory of fixed size for storing all autoencoders. We empirically demonstrate that our algorithm performs favorably compared to other state-of-art regularization-based continual learning methods.

==> algorithm_backup.tex <==
\begin{algorithm} %Complete Continual Learning algorithm
\caption{DCO Algorithm} % \caption should be before \label
\label{alg:continual_learning}
\begin{algorithmic}
\REQUIRE
% \STATE $\eta$ and $\eta_a$: learning rates of the model and autoencoders respectively. $\gamma_1, \gamma_2 \in (0,1]$: pulling strengths that controls the searching scope of the model parameters. 
% $N$: number of additional epochs used to train the model after saturation. $C$: number of points to average. $\theta$: step size for pushing the optimizer inside the cone ($\theta\leq1$ corresponds to parameter interpolation; $\theta>1$  corresponds to parameter extrapolation). 
% $m$: the size of the batch of gradients fed into autoencoders. $\tau$: the period of updates of the model parameters in step 3. 
$n$: number of tasks. $\mathcal{T}=\{\mathcal{T}_1, \dots, \mathcal{T}_n\}$: training data from task $1,2,\dots, n$. $|\mathcal{T}_i|$: number of iterations (mini-batches) required to process all data samples from task $i$.
\STATE 
\FOR{$i=1$ {\bfseries to} $n$}
% \STATE \# step 1: train model until convergence
% \STATE $x_0 \leftarrow x$
% \REPEAT
% \STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
% \STATE $x \leftarrow x - \eta \nabla_x L_i(x;\xi) - \gamma_1 (x - x_0)$ 
% \UNTIL convergence

% \STATE
% \STATE \# step 2: pushing the model parameters into the cone
% \STATE $x_1 \leftarrow 0, x_2 \leftarrow 0$
% \FOR{$j=1$ {\bfseries to} $N \times |\mathcal{T}_i|$}
% \STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
% \STATE $x \leftarrow x - \eta \nabla_x L_{ce}(x;\xi)$
% \STATE \bf{if} $j \leq C$ \bf{then} $x_1 \leftarrow x_1 + x$
% \STATE \bf{if} $j > N \times |\mathcal{T}_i| - C$ \bf{then} $x_2 \leftarrow x_2 + x$
% \ENDFOR
% \STATE $x^*_i \leftarrow x_1 - \theta\frac{(x_1-x_2)}{\norm{x_1-x_2}}$ \{push into the cone\}

% \STATE
% \STATE \# step 3: train autoencoder until convergence
% \REPEAT
% \STATE $g \leftarrow 0, G \leftarrow \{\}$
% \FOR{$j=1$ {\bfseries to} $m$}
% \STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
% \STATE $g \leftarrow g + \nabla_x L_{ce}(x;\xi)$; $G \leftarrow G \cup \nabla_x L_{ce}(x;\xi)$
% \IF {$\tau$ divides $j$}
% \STATE $x \leftarrow x - \eta g$; $g \leftarrow 0$
% \ENDIF
% \ENDFOR
% \STATE $G \leftarrow \frac{G}{\sqrt{\norm{G}_2^2/ m}}$ \{Normalize batch of gradients\}
% \STATE $W \leftarrow W - \frac{\eta_a}{m} \nabla_W L_{mse}(W;G)$; $x \leftarrow x - \gamma_2 (x - x_i^*)$
% \UNTIL convergence
% \STATE $W_i \leftarrow W$ \{Store autoencoder parameters\}
% % \STATE $x \leftarrow x_i^*$ \{Restore model parameters\}
\ENDFOR
\STATE \textbf{Output} $x_n^*$
\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{Train model}
\label{alg:push_cone}
\begin{algorithmic}
\REQUIRE $\eta$ and $\eta_a$: learning rates of the model and autoencoders respectively. $\gamma_1 \in (0,1]$: pulling strength that controls the searching scope of the model parameters. $\mathcal{T}_i$: training data.
\STATE \hspace*{-1.25em} \textbf{Input:} Initial model parameters $x_0$. 
\REPEAT
\STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
\STATE $x \leftarrow x - \eta \nabla_x L_i(x;\xi) - \gamma_1 (x - x_0)$ 
\UNTIL convergence
\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{Push model parameters into the cone}
\label{alg:push_cone}
\begin{algorithmic}
\REQUIRE $\eta$: learning rate of the model. $N$: number of additional epochs used to train the model after saturation.  $C$: number of points to average. $\theta$: step size for pushing the optimizer inside the cone. $\mathcal{T}_i$: training data.
\STATE \hspace*{-1.25em} \textbf{Input:} Model parameters $x$. 
% \STATE \hspace*{-1.25em} \textbf{Procedure:}
% \STATE 
\STATE $x_1 \leftarrow 0, x_2 \leftarrow 0$
\FOR{$j=1$ {\bfseries to} $N \times |\mathcal{T}|$}
\STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
\STATE $x \leftarrow x - \eta \nabla_x L_{ce}(x;\xi)$
\STATE \bf{if} $j \leq C$ \bf{then} $x_1 \leftarrow x_1 + x$ 
\STATE \bf{if} $j > N \times |\mathcal{T}| - C$ \bf{then} $x_2 \leftarrow x_2 + x$ 
\ENDFOR
\STATE $x^* \leftarrow x_1 - \theta\frac{(x_1-x_2)}{\norm{x_1-x_2}}$ \{push into the cone\}
\STATE \hspace*{-1.25em} \textbf{Output:} $x^*$
\end{algorithmic}
\end{algorithm}

\begin{algorithm} %Complete Continual Learning algorithm
\caption{Train autoencoder} % \caption should be before \label
\label{alg:train_autoencoder}
\begin{algorithmic}
\REQUIRE $\eta$ and $\eta_a$: learning rates of the model and autoencoders respectively. $\gamma_2 \in (0,1]$: pulling strength that controls the searching scope of the model parameters. $\mathcal{T}_i$: training data.
\STATE \hspace*{-1.25em} \textbf{Input:} Model parameters $x$ and initial autoencoder parameters $W$. 
\REPEAT
\STATE $g \leftarrow 0, G \leftarrow \{\}$
\FOR{$j=1$ {\bfseries to} $m$}
\STATE $\xi \leftarrow$ randomly sample from $\mathcal{T}_i$
\STATE $g \leftarrow g + \nabla_x L_{ce}(x;\xi)$; $G \leftarrow G \cup \nabla_x L_{ce}(x;\xi)$
\STATE \bf{if} {$\tau$ divides $j$} \bf{then} $x \leftarrow x - \eta g$; $g \leftarrow 0$
\ENDFOR
\STATE $G \leftarrow \frac{G}{\sqrt{\norm{G}_2^2/ m}}$ \{Normalize batch of gradients\}
\STATE $W \leftarrow W - \frac{\eta_a}{m} \nabla_W L_{mse}(W;G)$; $x \leftarrow x - \gamma_2 (x - x_i^*)$
\UNTIL convergence
\STATE \hspace*{-1.25em} \textbf{Output:} $W$
\end{algorithmic}
\end{algorithm}
